The Teichm\"uller space of the Hirsch foliation

We prove that the Teichm\"uller space of the Hirsch foliation (a minimal foliation of a closed 3-manifold by non-compact hyperbolic surfaces) is homeomorphic to the space of closed curves in the plane. This allows us to show that that the space of hyperbolic metrics on the foliation is a trivial principal fiber bundle. And that the structure group of this bundle, the arc-connected component of the identity in the group of homeomorphisms which are smooth on each leaf and vary continuously in the smooth topology in the transverse direction of the foliation, is contractible.

==> conformalpants.tex <==
The point of this section is to establish that any two equivalent hyperbolic metrics with geodesic boundaries on the pair of pants $P$ determine a canonical diffeomorphism which is isotopic to the identity and is an isometry between the two metrics.  This follows from the well known fact that any hyperbolic pair of pants can be split into two congruent hyperbolic hexagons though we will not prove it this way.  Instead we base our proof on the existence of a unique conformal hyperbolic metric on each planar pair of pants which allows us to obtain (from basic facts on the Beltrami equation) that the diffeomorphism depends continuously on the metrics in the smooth topology.  This also yields an essentially unique conformal model for each point in the Teichmüller space of a pair of pants.

\subsection{Conformal metrics and Teichmüller space}

In the following theorem, by a \emph{planar pair of pants} we mean any closed euclidian disk minus two open euclidian disks, whose closures are strictly included in its interior.  We continue to denote by $P$ the standard pair of pants $\lbrace |z| \le 1, |z\pm 1/2| \ge 1/4\rbrace$.

The following theorem establishes that the Teichmüller space $T(P)$ of the pair of pants $P$ is homeomorphic to the space of planar pairs of pants considered up to Möbius tranformations.

\begin{theorem}[Conformal models of Teichmüller space]
\label{conformalpantstheorem}
\begin{enumerate}
 \item Every planar pair of pants admits a unique conformal hyperbolic metric with geodesic boundaries.
 \item If $f:Q \to Q'$ is an isometry between the conformal hyperbolic metrics on two planar pairs of pants $Q$ and $Q'$ then $f$ is the restriction of a Möbius tranformation.
 \item Every hyperbolic metric with geodesic boundary components $g \in H(P)$ is isometric to the conformal hyperbolic metric on some planar pair of pants.  Furthermore, the isometry (and hence the resulting planar pair of pants) can be chosen to depend continuously on the metric $g$.
\end{enumerate}
\end{theorem}
\begin{proof}
Let $Q$ be a planar pair of pants.  To establish the first claim we apply Berger's work \cite{Berger1971} to the double of $Q$. More precisely, consider the reflections $R_1,R_2,R_3$ with respect to the three boundary components. The group $\Gamma_0$ whose elements are compositions of an even number of $R_i$ is a Kleinian group of $\C\PP^1$ whose limit set is a spherical Cantor set $K$. The quotient $(\C\PP^1\moins K)/\Gamma_0$ is identified with a genus two surface $S$. Since $\Gamma_0$ consists of conformal elements, $S$ inherits naturally a conformal structure from the one on $\C\PP^1$.
 
By \cite{Berger1971} there exists a unique hyperbolic metric in this conformal class denoted by $g_0$. Hence if $g$ is a conformal hyperbolic metric on $Q$ with geodesic boundary, it extends to a metric on $\C\PP^1\moins K$ which is $G$-invariant: the quotient metric is $g_0$: this gives the uniqueness.

Conversely the metric $g_0$ lifts to $\C\PP^1\moins K$ as a conformal hyperbolic metric denoted by $g$. For $i=1,2,3$ the reflection $R_i$ is anticonformal so that the pullback metric $R_i^{\ast}g$ is again hyperbolic, conformal, and it is easy to see that it is still $\Gamma_0$-invariant (since for every $\gamma\in \Gamma_0$, $R_i\gamma R_i\in \Gamma_0$, we have $(R_i\gamma R_i)^{\ast}g=g$, and $R_i^{\ast}g$ is $\gamma$-invariant). Hence it descends to the quotient and the quotient metric has to be $g_0$. This proves that $R_i^{\ast}g=g$ or, if one prefers, that $R_i$ is an isometry for $g$. Hence the boundary circles are geodesics: this gives the existence.

For the second claim suppose $f:Q \to Q'$ is an isometry between the conformal hyperbolic metric on $Q$ and that of $Q'$.  The function $f$ has a unique maximal extension satisfying $f\circ R = R'\circ f$ for every pair of reflexions $R,R'$ with respect to corresponding boundary components of $Q$ and $Q'$.  This extension is conformal outside of the Cantor set $K_Q$ which is the limit set of the group generated by reflexions with respect to the boundaries of $Q$.  Furthermore one can verify that $f$ extends continuously to $K_Q$ and, since $K_Q$ has zero one dimensional Hausdorff measure one obtains that $f$ extends conformally to the entire Riemann sphere by Painlevé's theorem (e.g. see \cite[Theorem 2.7]{dudziak2010}).

For the last claim consider a hyperbolic metric $g = E dx^2+2F dxdy+G dy^2$ on $P$ for which the boundary circles are geodesics and extend the Beltrami coefficient
\[\mu=\frac{E-G+2\ii F}{E+G+2\sqrt{EG-F^2}}\]
to the entire plane so that it satisfies
\[\mu\circ R = \frac{\partial_{\bar{z}}R}{\overline{\partial_{\bar{z}}R}}\bar{\mu}\]
for each reflexion $R$ with respect to a boundary of $P$ (the value of $\mu$ on the Cantor set $K_P$ can be chosen arbitrarily, for example to be $0$).

One can verify that $\mu$ is bounded so that there is a unique solution $f:\C \cup \lbrace \infty\rbrace \to \C \cup \lbrace \infty\rbrace$ to the Beltrami equation
\[\partial_{\bar{z}}f=\mu\partial_z f\]
which fixes $\infty$.  It follows from \cite[Lemma 2]{Sibner1965} that $f$ maps the boundary circles of $P$ to circles.   And, since $\mu$ is smooth outside of $K_P$ one has that $f$ is a smooth diffeomorphism from $P$ onto its image and depends continuously on $g$ (see \cite[Lecture 5]{Be}).  Hence $f(P) = Q$ is a planar pair of pants.  The pushforward metric $f_*g$ is conformal on $Q$ and hence must be the unique conformal hyperbolic metric for which the boundary circles of $Q$ are geodesics.
\end{proof}

\subsection{Canonical diffeomorphisms between metrics}

We will use the following consequence of Theorem \ref{conformalpantstheorem}.
\begin{lemma}\label{canonicaldiffeoslemma}
There exists a continuous function associating to each pair of equivalent metrics $g,g' \in H(P)$ a self-diffeomorphism $f:P \to P$ isotopic to the identity such that $f_*g = g'$.
\end{lemma}
\begin{proof}
The result follows by setting $f = f_{g'}^{-1} \circ h \circ f_g$ where $f_g$ and $f_{g'}$ are obtained by solving Beltrami's equation as in Theorem \ref{conformalpantstheorem} and map $P$ onto planar pants $Q$ and $Q'$ respectively, and $h:Q \to Q'$ is the unique Möbius transformation between $Q$ and $Q'$ such that $f$ preserves the each boundary component of $P$.
\end{proof}

==> deforminggeeodesicmeridians.tex <==
We have previously produced for each pair of functions $\lambda:S^1 \to \R^+$ and $\tau:S^1 \to \R$ a hyperbolic metric $g_{\lambda,\tau}$ on the Hirsch foliation and have shown that distinct pairs of functions correspond to distinct hyperbolic metrics (where equivalence is up to identity isotopies which preserve the leaves and are smooth on each leaf).

What remains of the article is dedicated to proving that any hyperbolic metric on the Hirsch foliation is equivalent to some $g_{\lambda,\tau}$.

By a meridian of the Hirsch foliation we mean the projection of any curve of the form $\lbrace e^{it}\rbrace \times S^1 \subset S^1 \times \C$.  Notice that for the metrics $g_{\lambda,\tau}$ all geodesics are meridians.   In this subsection we will consider only metrics for which this is the case, proving the following:
\begin{proposition}
\label{geodesicmeridians}
Let $g$ be a hyperbolic metric on the Hirsch foliation for which all meridians are geodesics.  Then $g$ is equivalent to $g_{\lambda,\tau}$ for a unique choice of $\lambda:S^1 \to \R^+$ and $\tau:S^1 \to \R$.
\end{proposition}

Before we carry on the proof of this proposition, let us remark that the uniqueness of the length and twist functions follow from Theorem \textbf{BLA}.

\subsection{Path in restriction to a fundamental domain}

A hyperbolic metric on the Hirsch foliation $g$ can be lifted to $(S^1\times\C)\moins K$ as a foliated metric, still denoted by $g$, which is $f$-invariant. 

Consider the fundamental domain $D=\bigcup_{t} P_t$ (see the notations of Section \textbf{bla}). If we ask the meridians to be geodesics for $g$, then the fundamental domain $D$ has ``geodesic boundaries'' in the sense that for every $t$, $\partial P_t$ is geodesic.

Say that a hyperbolic metric $g$ on the Hirsch foliation is \emph{admissible} if all the meridians are geodesics, and if the lifted metric is admissible in restriction to the pairs of pants $P_t$.

The first step of the proof is to reduce the study to the case of admissible metrics.

\begin{lemma}
\label{admissible}
Let $g$ be a hyperbolic metric on the Hirsch foliation for which all meridians are geodesics. Then $g$ is equivalent to an admissible hyperbolic metric.
\end{lemma}

\begin{proof}
Let $g$ be such as in the statement of the lemma: lift it to $(S^1\times\C)\moins K$.

Now we can apply the isotopy $F_{t,g_t}$ in the annular neighbourhood $S^1\times\A$ (see the notation of Paragraph \textbf{BLA}), as well as the corresponding isotopies in the image by $f^k$ of this annular neighborhood (they are all disjoint). By doing so, we obtain an leafwise identity isotopy of $(S^1\times\C)\moins K$ which is $f$-invariant, and which provides a path between $g$ and some admissible metric, concluding the proof of the lemma.
\end{proof}

Consider such an admissible metric $g$ and denote $g_t=g_{|P_t}$. Let $\lambda(e^{it})$ be the length for $g_t$ of the outer boundary of $P_t$ and define $ \mg=(\mg_t)_t$ as the family of metrics compatible with $\lambda$ which is used in the construction of all $g_{\lambda,\tau}$ (see Section \textbf{bla}).

By Theorem \ref{canonicaldiffeo}, for every $t$, we have a diffeomorphism $\phi_t:P_t\to P_t$ isotopic to the identity which varies continuously in the smooth topology and such that $(\phi_t)_{\ast}g_t = \mg_t$ for all $t$.

We now use the fact that the space of diffeomorphisms of $P$ isotopic to the identity is contractible and this coincides with the set of diffeomorphisms which preserve the three boundary components (see \cite[Theorem 2.10]{FLP}). Fixing a contraction and applying it to $\phi_t$ yields an isotopy $\phi_t^s:P_t\to P_t$ between $\phi_t$ and the identity, which varies continuously in the $C^{\infty}$-topology with respect to $t$.

We then have a continuous homotopy $\Phi^s:D\to D$ which coincides with $\phi_t^s$ when restricted to $P_t$ and provides a path between $g^0=g_{|D}$ and $g^1=\mg$.

\subsection{Passing through admissible metrics} 

In order to recover the twist parameter, it is useful to project this path of metrics via the map $F$ constructed in Section \textbf{BLA} so as to deal with admissible metrics.

The map $F$ defined in Section \textbf{BLA} clearly provides a map of foliated hyperbolic metrics on $D$, still denoted by $(t,g)\mapsto F(t,g)$, where $t\in[0,1]$ and $g$ is a foliated hyperbolic metric on $D$.

\begin{lemma}
\label{passingthroughadm}
There exists a continuous homotopy $\Psi:D\times[0,1]\to D$ which is an identity isotopy when restricted to each $P_t$ such that:
\begin{enumerate}
\item $\Psi^1_{\ast}g^0=g^1$;
\item for every $s\in[0,1]$, $g^s=\Psi^s_{\ast}g^0$ is admissible.
\end{enumerate}
\end{lemma}

\begin{proof}
Assume that we have a path $g^s$ of admissible foliated hyperbolic metrics on $D$ between $g^0$ and $g^1$. Then Corollary \ref{pathmetrics} clearly provides the foliated isotopy $\Psi^s:D\times [0,1]\to D$ . Hence, it is enough to provide this continuous path of foliated metrics.


Consider the foliated metrics $\widehat{g}^s=\Phi^s_{\ast}g^0$. This provides a path of foliated hyperbolic metrics between $g^0$ and $g^1$, but which passes a priori through nonadmissible metrics. But $F(1,\widehat{g}^s)$ provides a path between $F(1,g^0)$ and $F(1,g^1)$ through admissible metrics.

But since for $\star=0,1$, $g^{\star}$ is admissible, $F(s,g^{\star})$ is admissible for $s\in[0,1]$. Concatenating these three paths, we obtain the desired path of foliated hyperbolic metrics.
\end{proof}

%\begin{lemma}
%\label{extend}
%Let $\tau:S^1\to\R$ be a continuous function. Then, for $s\in[0,1]$ there is an extension $F_{\tau}(s,.)$ of $F(s,.)$ to $(S^1\times\C)\moins K_{\tau}$ such that for every $g$ foliated hyperbolic on $(S^1\times\C)\moins K_{\tau}$ which is $f_{\tau}$-invariant, the foliated hyperbolic metric $F_{\tau}(s,g)$ is $f_{\tau}$-invariant.
%\end{lemma}
%
%\begin{proof}
%This follows directly from Lemma \ref{affineinvariance}.
%\end{proof}
%
%Inside $D$, consider the family  $\widehat{g}^s=F(1,g^s)$. This gives a continuous path between leafwise admissible hyperbolic metrics on $D$. Moreover, by Lemma \ref{extend}, $\widehat{g}^0$ extends as a $f$-invariant metric on $S^1\times\C\moins K$.
%
%Composing the homotopy $\Phi^s$ by $F$, one obtains a new homotopy  $\widehat{\Phi}^s$ of $D$ which is a identity isotopy when restricted to $P_t$, and satisfy $(\widehat{\Phi}^s)_{\ast}\widehat{g}^0=\widehat{g}^s$.

\subsection{Extending the foliated isotopy}

\begin{lemma}
\label{extendadmissible}
There exists a family of continuous functions $\tau_s:S^1\to\R$ such that each $\Psi^s$ extend to a homeomorphism of $(S^1\times\C)\moins K_{\tau_s}$ such that $\tau_0=0$ and which satisfies the following relation of equivariance:
\begin{equation}
\label{equivariance}
\Psi^s\circ f=f_{\tau_s}\circ \Psi^s.
\end{equation}
\end{lemma}

\begin{proof}
Notice that since each $g_t^s$ is admissible one has that $\Psi_t^s$ must be a rotation on a neighborhood of each boundary of $P_t$.  Hence there exists for each $s \in [0,1]$ a twist parameter $\tau_s:S^1 \to \R$ such that $\tau_0 = 0$ and Relation \ref{equivariance} holds.
\end{proof}

Now, notice that since $g$ is $f$-invariant and coincide with $g_0$ in $D$, if we push $g$ by $\Psi^s$ we get a path of metrics $g^s$ on $(S^1\times\C)\moins K_{\tau_s}$ which are $f_{\tau_s}$-invariant.


\paragraph{End of the proof of Proposition \ref{geodesicmeridians}}

Consider $\tau=\tau_1$. We remarked that the foliated metric $g^1=\Psi^1_{\ast}g$ is the foliated hyperbolic metric on $(S^1\times\C)\moins K_{\tau}$ which is $f_{\tau}$-invariant and coincide with $\mg$ inside $D$.

But as we noted in Section \textbf{BLA}, by pushing by an appropriate $h_{\tau}$, an $f_{\tau}$-invariant leafwise hyperbolic metric on $(S^1\times\C)\moins K_{\tau}$ provides an $f$-invariant leafwise hyperbolic metric on $(S^1\times\C)\moins K$, and hence a leafwise hyperbolic metric on the Hirsch foliation.

Hence, the path we just described provides a leaf-preserving isotopy sending the original metric $g$ onto $g_{\lambda,\tau}$ where $\lambda$ and $\tau$ have been described in the previous paragraphs. This concludes the proof of Proposition \ref{geodesicmeridians}.\quad \hfill $\square$


==> generalmetrics.tex <==
blah blah

==> geodesicmeridians.tex <==
We have previously produced for each pair of functions $\lambda:S^1 \to \R^+$ and $\tau:S^1 \to \R$ a hyperbolic metric $g_{\lambda,\tau}$ on the Hirsch foliation and have shown that distinct pairs of functions correspond to distinct hyperbolic metrics (where equivalence is up to identity isotopies which preserve the leaves and are smooth on each leaf).

What remains of the article is dedicated to proving that any hyperbolic metric on the Hirsch foliation is equivalent to some $g_{\lambda,\tau}$.

By a meridian of the Hirsch foliation we mean the projection of any curve of the form $\lbrace e^{it}\rbrace \times S^1 \subset S^1 \times \C$.  Notice that for the metrics $g_{\lambda,\tau}$ all geodesics are meridians.   In this subsection we will consider only metrics for which this is the case, proving the following:
\begin{lemma}
Let $g$ be a hyperbolic metric on the Hirsch foliation for which all meridians are geodesics.  Then $g$ is equivalent to $g_{\lambda,\tau}$ for a unique choice of $\lambda:S^1 \to \R^+$ and $\tau:S^1 \to \R$ (.
\end{lemma}
\begin{proof}
The uniqueness claim follows immediately from Lemma \ref{fenchelnielseninjectivity}.  Furthermore, applying the proceedure of Section \ref{admissiblehomotopy} in an annulus around each meridian we may assume that, when lifted to $S^1 \times \C$ the metric is standard on each pair of pants $P_t \subset \lbrace e^{it}\rbrace \times \C$.

Let $g_t^0$ be the lift of the given hyperbolic metric $g$ to $P_t$ (which we assume standard).  Let $\lambda(e^{it})$ be the length for $g_t$ of the outer boundary of $P_t$ and define $g_t^1$ as the family of metrics compatible with $\lambda$ which is used in the construction of all $g_{\lambda,\tau}$ (see Section \ref{standardmetrics}).

By Lemma \ref{canonicaldiffeoslemma} there exists a family of diffeomorphisms $f_t:P_t \to P_t$ isotopic to the identity which varies continuously in the smooth topology and such that $(f_t)_{*}g_t^0 = g_t^1$ for all $t$.

Notice that the space of diffeomorphisms of $P$ isotopic to the identity is contractible and this coincides with the set of diffeomorphisms which preserve the three boundary components (see \cite[Theorem 2.10]{FLP}).   Fixing a contraction yields a continuous path $s \mapsto f_t^s$ (where $s \in [0,1]$) the identity to $f_t$ for each $t$, which varies continuously with respect to $t$.  Define for each $s,t$ the metric $\hat{g}_t^s = (f_t^s)_*g_t^0$.  This yields a path of metrics between $g_t^0$ and $g_t^1$.  We project this path onto the admissible metrics $A(P)$ using the mapping $F_1$ obtained in Theorem \ref{admissiblehomotopy} which yields a path $g_t^s$ (where $s \in [0,1]$) between $g_t^0$ and $g_t^1$ consisting only of admissible metrics and which varies continuously with respect to $t$.

Finally for each $s,t$ define $f_t^s$ the diffeomorphism given by Lemma \ref{canonicaldiffeoslemma} of $P_t$ sending $g_t^0$ to $g_t^s$.

Notice that since each $g_t^s$ is admissible one has that $f_t^s$ must be a rotation on a neighborhood of each boundary of $P_t$.  Hence there exists for each $s \in [0,1]$ a twist parameter $\tau_s:S^1 \to \R$ such that $\tau_0 = 0$ and the family $f_t^s$ can be extended to be $f_{\tau_s}$ periodic (recall the twisted solenoid map $f_\tau$ defined in Section \ref{standardmetrics}).  Therefore for each $s$ one has a well defined self homeomorphism $F_s$ of $(S^1 \times \C) \setminus K_\tau$ which is $f_{\tau_s}$ periodic.

A leaf preserving identity isotopy of the Hirsch foliation is obtained as the projection of $H_s = h_{\tau_s}^{-1}\circ F_s\circ h_{\tau_s}$.  For each $s$ the pushforward of the original hyperbolic metric under $H_s$ is the family $g_t^s$ on each pair of pants $P_t$ in the lift.   For $s = 1$ one obtains the pullback of the family $g_t^1$ under $h_{\tau_1}$ which is exactly the definition of $g_{\lambda,\tau_1}$. Tje issue is now to know how to glue them together. For this purpose, it will be convenient to project this path to admissible metrics by the isotopy $F$ constructed .

Consider $H:[0,3]\times A(D)\to A(D)$ such that for every $g\in 
\begin{itemize}
\item $H$ and $F$
\item 
\item 
\end{itemize}


\end{proof}



==> hirsch.tex <==
\subsection{The Hirsch foliation}

Consider the smooth endomorphism $f$ of $S^1\times \C$ (where $S^1 = \lbrace z \in \C: |z|=1\rbrace$) defined by
\[f(e^{it},z) = \left(e^{i2t},\frac{1}{2}e^{it} + \frac{1}{4}z\right).\]

Let $T = S^1 \times \D$ (where $\D$ is the open unit disk).  The closed solid torus $\overline{T}$ is mapped diffeomorphically into $T$ by $f$.  In fact, $f$ restricted to $\overline{T}$ is the well known solenoid map and the compact set $K_0 = \bigcap\limits_{n \ge 0}f^{n}(\overline{T})$ is a hyperbolic attractor which is locally homeomorphic to $\R$ times a Cantor set.   

Let $K$ be the union of preimages of $K_0$.  The quotient $M = ((S^1 \times \C) \setminus K)/f$ (where two points $x,y$ are equivalent if they belong to the same complete orbit, i.e. if $f^n(x) = f^m(y)$ for some $n,m \ge 0$) is a compact boundaryless smooth manifold and the foliation of $(S^1 \times \C) \setminus K$ by leaves of the form $\lbrace e^{it}\rbrace \times \C \setminus K$ descends to $M$.   The resulting foliated compact boundaryless $3$-manifold (where both the manifold and the leaves of the foliation are smooth) is what we will call from now on the Hirsch foliation. $(M,\F)$.

One can verify that each complete $f$-orbit intersects $\overline{T} \setminus f(T)$ (which is a $3$-manifold with two boundary components which are $2$-dimensional tori) at exactly one interior point or at one point on each boundary component.  Hence $M$ is obtained by pasting the two boundaries of $\overline{T} \setminus f(T)$ using $f$.  The sets of the form $P_t = \overline{T} \setminus f(T) \bigcap \lbrace e^{it}\rbrace \times \C$ are pairs of pants, and the partition of $\overline{T} \setminus f(T)$ into these pants when pasted using $f$ yields the Hirsch foliation.  With this description it is simple to see that the leaves of the Hirsch foliation are homeomorphic to either the the two-dimensional torus minus a Cantor set or the two-dimensional sphere minus a Cantor set (depending on whether the leaf contains a pair of pants $P_t$ such that $e^{it}$ is periodic under iterated squaring or not).

\subsection{Teichmüller space of the Hirsch foliation}

A hyperbolic metric on the Hirsch foliation is an assignment of a smooth hyperbolic Riemannian metric to each leaf which when lifted to an $f$-invariant family $g_t$ of metrics on $\lbrace e^{it}\rbrace \times \C \setminus K$ vary continuously with respect to $t$ in the topology of smooth convergence on compact subsets of $\C$.  The existence of hyperbolic metrics on the Hirsch foliation follows from the results of \cite{Candel} on uniformization of foliations.
\begin{theorem}[Candel]\label{candelstheorem}
There exists at least one hyperbolic metric on the Hirsch foliation.
\end{theorem}

We denote by $H(M,\F)$ the set of hyperbolic metrics on the Hirsch foliation endowed with the topology of locally uniform leafwise smooth convergence.

A identity isotopy on the Hirsch foliation is a continuous function $F:[0,1] \times M \to M$ which satisfies the following
\begin{enumerate}
 \item For each $s \in [0,1]$ the function $F_s$ is a homeomorphism of $M$.
 \item For each $s \in [0,1]$ the function $F_s$ is a smooth self diffeomorphism when restricted to any leaf of the Hirsch foliation.
 \item When $F$ is lifted to $(S^1 \times \C) \setminus K$ the resulting restriction to sets of the form $\lbrace (e^{it} \times \C) \times K$ vary continuously with respect to $t$ in the topology of smooth convergence on compact subsets.
\end{enumerate}

Given a hyperbolic metric $g$ on the Hirsch foliation and an identity isotopy $F$ one may push forward or pull back the metric $g$ using $F_s$ to obtain a curve of metrics in $H(M,\F)$.  Any two metrics which belong to such a curve are considered equivalent and the resulting quotient space $T(M,\F) = H(M,\F)/\sim$ is the Teichmüller space of the Hirsch foliation.

Our main result is the identification of $T(M,\F)$ up to homeomorphism.
\begin{theorem}\label{hirschteichmuller}
The Teichmüller space of the Hirsch foliation is homeomorphic to the space of pairs of continuous functions $(\lambda,\tau)$ where $\lambda:S^1 \to \R^+$ and $\tau:S^1 \to \R$, endowed with the topology of uniform convergence.
\end{theorem}

The functions $\lambda$ and $\tau$ can be considered to be Fenchel-Nielsen coordinates for Teichmüller space.  In particular the values of $\lambda$ represent lengths of closed geodesics and those of $\tau$ represent a twist parameter.

\subsection{Standard metrics on the Hirsch foliation\label{standardmetrics}}

As a first step to prove Theorem \ref{hirschteichmuller}, given a continuous length function $\lambda:S^1 \to \R^+$ and a continuous twist function $\tau:S^1 \to \R$ we will construct a hyperbolic metric on the Hirsch foliation.

First fix a global section of the Teichmüller space $T(P)$ of the pair of pants $P$ by admissible metrics (this is possible due to Theorem \ref{admissibleglobalsection}).  Each pair of pants $P_t \subset S^1 \times \C$ can be identified with $P$ via projection onto the second coordinate followed by a rotation $z \mapsto e^{-it/2}z$ (of course $P_t = P_{t+ 2\pi}$ but the identifications to $P$ defined using $t$ and $t+2\pi$ are not the same, one can check that what follows is unaffected by this ambiguity).   On $P_t$ we consider the metric coming from the global section just chosen such that the outer boundary (the one corresponding to $S^1$ under the identification with $P$) has length $\lambda(e^{it})$ and the other two have lengths $\lambda(e^{it/2})$ and $\lambda(e^{i(t+2\pi)/2})$ according to whether their preimages under $f$ belong to $P_{t/2}$ or $P_{(t+2\pi)/2}$.  Let $g_t$ be the thus chosen metric on $P_t$.

Consider the map $f_\tau:S^1 \times \C \to S^1 \times \C$ defined by
\[f_\tau(e^{it},z) = \left(e^{i2t},\frac{1}{2}e^{it} + \frac{e^{i\tau(e^{it})}}{4}z\right).\]

Because the metric $g_t$ is admissible, its pushforward under $f_\tau$ (which is defined on a subset of $\lbrace e^{i2t}\rbrace \times \C$ contained in one of the `holes' of the pair of pants $P_{2t}$) coincides with $g_{2t}$ where both are defined.  Furthermore,  both metrics are standard around the circle where they intersect and therefore glue together smoothly.   Hence one may extend the family $g_t$ to a unique maximal $f_\tau$-invariant family of metrics on $(S^1 \times \C) \setminus K_\sigma$ where $K_\sigma$ is defined analogously to $K$ replacing $f$ by $f_\sigma$.

The map $f_\tau$ depends on the twist parameter $\tau$ only up to multiples of $2\pi$.  However we will choose a conjugating homeomorphism $h_\tau$ which depends on the actual values of $\tau$.   The homeomorphism $h_\tau$ is defined by the following as the homeomorphism satisfying the following properties
\begin{enumerate}
 \item The map is of the form $h_\tau(e^{it},z) = (e^{it}, h_{\tau,t}(z))$.
 \item For each $t$ the map $h_{\tau,t}$ coincides with $z \mapsto e^{-i\rho(|z|)\tau(e^{it})}z$ on the pair of pants $P_t$, where $\rho$ is the step function of section \ref{auxiliarystep}.
 \item One has $f\circ h_\tau = h_\tau \circ f_\tau$ on all of $S^1 \times \C$.
\end{enumerate}

Pushing forward the metrics $g_s$ using $h_\tau$ one obtains an $f$ invariant family of metrics on $(S^1 \times \C) \setminus K$ and hence a hyperbolic metric on the Hirsch foliation $g_{\lambda,\tau}$.

We now show that this construction yields infinitely many non-equivalent hyperbolic metrics.
\begin{lemma}\label{fenchelnielseninjectivity}
If $g_{\lambda,\tau}$ belongs to the same Teichmüller equivalence class as $g_{\lambda',\tau'}$ then $\lambda = \lambda'$ and $\tau = \tau'$.
\end{lemma}
\begin{proof}
Let $g_t$ and $g_t'$ be the family of metrics on the sets $\C_t = (\lbrace e^{it}\rbrace \times \C) \setminus K$ obtained by lifting $g_{\lambda,\tau}$ and $g_{\lambda',\tau'}$ to $(S^1 \times \C)\setminus K$.

Suppose there is an leaf preserving identity isotopy taking $g_{\lambda,\tau}$ to $g_{\lambda',\tau'}$.  Then lifting it one obtains an identity isotopy $F:[0,1] \times (S^1\times \C) \setminus K \to (S^1\times \C) \setminus K$ which preserves each $\C_t$ and such that $F_1$ sends $g_t$ to $g_t'$.

Since the outer boundary $C_t$ of the pair of pants $P_t$ is the unique closed geodesic in its isotopy class on its leaf for both $g_t$ and $g_t'$, one must have $F_1(C_t) = C_t$.  This implies that the length of $C_t$ is the same for both $g_t$ and $g_t'$ and since this is valid for all $t$ one obtains $\lambda = \lambda'$.

To show that $\tau = \tau'$ we first observe that any hyperbolic pair of pants with geodesic boundary components can be split in a unique way into two congruent hyperbolic right-angled hexagons.  This gives us a canonically defined pair of points which split each geodesic boundary comoponent in two.  If $g_{\lambda,\tau}$ and $g_{\lambda,\tau'}$ are equivalent then the angle between the thus obtained pairs of points on the boundaries of two neighboring pairs of pants in the foliation must coincide for both metrics.  This yields that there must exist an integer $n$ such that $\tau(e^{it}) - \tau'(e^{it}) = 2\pi n$ for all $t$.

To conclude the proof we will show that $n = 0$.  To see this consider the leaf containing the pair of pants $P_1 = \lbrace 1\rbrace \times P$.  

Notice that $P_1$ projects to a torus minus a disk $S$ in the foliation and that both metrics coincide on $S$.  Since $f_\tau = f_{\tau + 2\pi n} = f_{\tau'}$ one obtains that the map $h = h_{\tau'}^{-1}\circ h_{\tau}$ commutes with $f$ and hence projects to a leaf preserving homeomorphism $H$ of the Hirsch foliation.  If $\tau \neq \tau'$ then $H$ is a Dehn twist on $S$ of angle $2\pi n$.  On the other hand $H$ is an between the hyperbolic metrics $g_{\lambda,\tau}$ and $g_{\lambda,\tau'}$ on $S$.   Because both metrics coincide one has that $H$ is an self-isometry of $S$ endowed with either one of them and hence has finite order.  This shows that $n= 0$ as claimed
\end{proof}
